Fantastyc: Blockchain-based Federated Learning Made Secure and Practical

Federated Learning is a decentralized framework that enables multiple clients to collaboratively train a machine learning model under the orchestration of a central server without sharing their local data. The centrality of this framework represents a point of failure which is addressed in literature by blockchain-based federated learning approaches. While ensuring a fully-decentralized solution with traceability, such approaches still face several challenges about integrity, confidentiality and scalability to be practically deployed. In this paper, we propose Fantastyc, a solution designed to address these challenges that have been never met together in the state of the art.

==> app_correctness.tex <==
%\adp{check what to leave in the main body and refer to the appendix}
%\section{Correctness arguments}\label{sec:proofs}
%\adp{Proofs on the PoIA. To prove that if a PoIA exists, then the data is eventually available and valid. On the other hand, prove that Byzantine processes alone cannot produce any PoIA if the data is not integer and available.\\
%Also add proofs on the f+1 and 2f+2.}
%%%%%%%%%%
In the following we discuss the correctness argument related to the solution detailed in Section \ref{sec:workflow}.


In the next we consider the following Assumption:
\begin{assumption}\label{ass:selectedClients}
    The set of clients that join an FL task is such that {\sf select\_clients} returns a set that contains less than half Byzantine clients, enough to produce sufficiently many updates at each round to compute the aggregation robust to Byzantine clients (as defined in Section~\ref{par:fedavg}).
\end{assumption}

With this assumption, we abstract the implementation of the selection function, assuming only that the selection is verifiable. In practice, the selection function can be secret to ensure resilience against an adaptive adversary that can choose which clients to corrupt, or it can be public if only a static adversary is assumed.\\

\subsection{Safety}

Let $C^C_t$ and $S^C$ be the set of selected correct clients at round $t$ and the set of correct servers respectively. 
\begin{lemma} (availability and integrity)\label{lem:poia}
    For any $({\tagtt}, v)$, if exists a valid $P({\tagtt},v)$, then ${{\sf locally\_valid}}({\tagtt}, v)$ holds for at least one correct server, and eventually, $v$ is available from the distributed storage. 
\end{lemma}

\begin{proof}[Sketch]
    In Algorithm \ref{algo:read}, a process invokes a {\sf read} operation either in {\sf GET} ({line \ref{algo-read-get}}) or in {\sf GETALL} ({line \ref{algo-read-getall}}) if the input is a \poia.
    By definition, a $P({\tagtt},v)$ contains $f_s+1$ different 
    signatures on the same hash-key $h(v)$. Hence, at least one correct server $p$ signed.
    $p$ executes line 27, Algorithm~\ref{algo:server}, if ${\sf locally\_valid}({\tagtt},v)$ holds and after 
    having sent $\langle h(v),v \rangle$, to all storage replicas (lines 22 and 24). 
    %
    (consequently, ${{\sf locally\_valid}}({\tagtt}, v)$ holds for at least one correct server among the servers that signed).
    Eventually, all correct replicas receive $\langle h(v),v \rangle$. As the hash of $v$ corresponds to the hash-key $h(v)$, correct replicas store it forever (it is not possible to modify it, e.g. sending $\langle h(v),v' \rangle$). 
    Let $r$ be the first correct replica that stores $\langle h(v),v \rangle$ and let $t$ be this time.
   
    Let $q$ be a correct process that given $P({\tagtt},v)$ queries the key-value store for $h(v)$ after $t$. $q$ executes line~\ref{algo-read-get}, Algorithm~\ref{algo:read}. After verifying the proof validity (line~\ref{algo-read-check}), $q$ invokes a {\sf read} operation over the storage, sending a QUERY message to all replicas (line~\ref{algo-read-request}) and returns as soon as he gets a value, whose hash corresponds to the requested one. We need to prove that the {\sf read} terminates.
    By assumption, there are $f_r+1$ replicas. 
    As line~\ref{algo-read-request} occurs after $t$, then at least $r$ receives the query message and replies with $v$ to $q$. 
    The {\sf read} returns as $p$ receives the replay $\ell'$ from $r$. As sent by $q$, the hash of $\ell'$ matches with the requested hash-key, so the {\sf read} returns $v$ at line \ref{algo-read-return}.%, which concludes the proof.
\end{proof}


\begin{theorem}(Safety)
    If a model ownerobtains a $w_{fin}$ then $w_{fin}$ is $\epsilon$-valid %(i.e. $\epsilon$-close to a model produced by a correct server using a robust aggregation function as defined in Section~\ref{par:fedavg}) 
    and issued from a sequence of only $\epsilon$-valid  models.
\end{theorem}
%\adp{add that the aggregation function is robust to byzantine clients. to be placed with assumption 2.}
\begin{proof}[Sketch]
    Each $C_t^C$ client computes an update from an aggregated model $w_{t-1}$ if $w_{t-1}$ possesses a PoA$\&$I (cf. step 4). Hence $w_{t-1}$ is $\epsilon$-valid (Lemma \ref{lem:poia}). 
    The proof concludes by extending the reasoning to the entire sequence of models produced during the FL task as each associated to a \poia.
\end{proof}

\subsection{Liveness}

\begin{lemma}\label{lem:poialiveness}
    For each $t\in [0, t_{fin}]$ (steps \ref{loop:first-step}-\ref{loop:last-step}), 
    each correct server has sufficiently many PoA$\&$I for ${(\tagtt, v)}, \tagtt\in \{\updtt, \modtt, \clientstt\}$ to terminate the round.
    %\footnote{Let us recall that the $REWARD$ messages are not specified in the pseudo-code, as issued just once at the end of the FL task, those are handled similarly to $\clientstt$ messages.}.
\end{lemma}

\begin{proof}[Sketch]
We start from round $t=0$: %, and proceed by construction:

\noindent{\bf-} $\updtt$: 
    At $t=0$, there is a sufficient number of clients in $C_t^C$ to produce the required updates for the next robust aggregation (Assumption~\ref{ass:selectedClients}). 
    By recording the hash-key of the initial model on-chain, the Model Owner (MO) allows each $k\in C_{t}^C$ to retrieve the model from storage, compute, and send the update $g_{t=0}^k$ to the servers.
    All $S^C$ servers, eventually receive such updates, which pass the ${\sf locally\_valid}$ check.
    Thus, all $p \in S^C$ send the same message $\langle(\lptt, \tagtt, h(g_{t=0}^k)_p)\rangle$ (modulo the signature) to all servers. Each $S^C$ server
    collects $f_s+1$ $(\langle\lptt, \tagtt, h(g_{t=0}^k)_p\rangle)$ and produces a \poia for each update issued by each $k\in C_{t}^C$.

\noindent{\bf-} $\clientstt$: The same reasoning as in the previous case applies. Indeed, $C_t$ is the result of the same deterministic computation at all $S^C$ servers (line 13) which all send $\langle \lptt, \clientstt, h(C_t)_p\rangle$ to all servers (line 28).
  
    
\noindent{\bf-} $\modtt$: From the $\updtt$ case and the Assumption~\ref{ass:selectedClients} it follows that eventually line \ref{algo-server-candidateset} Algorithm~\ref{algo:server} holds at each $p \in S^C$.
   $p$ executes line 13 to select the next client set and starts building the \poia for it (line 14).
    Given the $\clientstt$ case, eventually lines 35 and 39 hold for $\tagtt=\clientstt$, and $p$ executes line 40 sending a $\nrtt$ transaction on the blockchain carrying a candidate update set and the next client set.
    The first of those $\nrtt$ transactions on-chain triggers the execution of line 15 at each $p \in S^C$.
    $p$ retrieves the missing updates (if any) using  their \poia (line 19). $p$ computes the new aggregated model $w_p^{t}$, and builds a \poia for it.
    This implies that $w_p^t$ is sent to all other servers (cf. line 27).
    Upon its reception (line 29), line 30 holds at each correct server for Assumption~\ref{ass:epsilonmodels}. Thus, all $q \in S^C$s send $\langle \lptt, \modtt, h(w_p^t)_q\rangle$ (modulo the signature) to all servers.
    All $S^C$ servers receive $f_s+1$ messages to build a PoA$\&$I for $w_p^t$, which triggers the sending of the \poia model to clients and the computation to move to the next round (lines 43-44).


The difference for $t\in [1, t_{fin}]$ is from where clients get the model hash-key. From $t \geq 1$, the hash-key is provided by servers via its \poia (line 43). Once $C_t^C$ clients retrieve one of the $\epsilon$-valid $w_p^t$ the process proceeds as described for $t=0$. 
\end{proof}



\begin{theorem}(Liveness)
     If a model owner sets up an FL task, then eventually the model owner obtains a trained model.
\end{theorem}

\begin{proof}[Sketch]
   Through the iterative application of Lemma~\ref{lem:poialiveness} to each round, it is inferred that when the model ownerstarts an FL task, this progresses round after round. %We need to prove that the MO receives the \poia of the final trained model.
    As discussed in step \ref{loop:last-step} and in Algorithm~\ref{algo:server} at line 41, each server $p\in S^C$ knows when the training terminates. 
    Hence, $p$ produces a \poia for the rewarding information (similarly to the $\clientstt$ case in Lemma~\ref{lem:poialiveness}) and for the last model ($t_{fin}$ in Lemma~\ref{lem:poialiveness}).
    $p$ has all the elements to send the final transaction, which is eventually on-chain and accessible to the MO.
    % To prove that the task terminates we need to prove that the the waiting conditions in Algorithm \ref{algo:server} are eventually satisfied. Hence we need the following conditions to hold:
    % \begin{itemize}
    %     \item sufficiently many correct clients join the computation, so that the first $C_1$ can be computed and the first round can start $\Rightarrow$ directly from Assumption \ref{ass:selectedClients}.
    %     \item during each round:
    %         \begin{itemize}
    %             \item sufficiently many correct clients compute and send their updates to servers $\Rightarrow$ directly from Assumption \ref{ass:selectedClients}, considering that correct clients follow the protocol;
    %             \item Servers generate PoA$\&$I for the updates and the set of updates' PoA$\&$I, ensuring that at least one of them is recorded on-chain along with the selected clients for the next round $\Rightarrow$ the first part of the proof derives from Lemma \ref{lem:updates}. The second part, concerning the selected clients, follows the same logic as Lemma \ref{lem:updates}, considering that all correct servers compute the same client selection and are thus capable of producing a PoA$\&$I for it.
    %             \item If any server did not receive certain updates from the valid update set recorded on-chain directly from the client, it can retrieve them from the storage $\Rightarrow$ this hold considering that an update set if valid if each update is represented with its PoA$\&$I, which from Lemma \ref{lem:poia} implies that each server can get it from the distributed storage.
    %             \item servers produce the aggregated models such that at least one of those obtains a PoA$\&$I, which is diffused to clients $\Rightarrow$ the proof follows from Assumption \ref{ass:epsilonmodels}
    %         \end{itemize}
    % \end{itemize}
\end{proof}
   


==> app_sequence.tex <==
%\adp{Introduce the sequence diagram and update it and refer to the appendix in the main body}
Fig. \ref{fig:sequence diagram} details the workflow described in Section \ref{sec:workflow}, involving replicated servers, storage replicas, a blockchain, clients, and a model owner. In particular, we use a replicated activation box image on the server lifeline, corresponding to the {\sf build PoA$\&$I} operation. With some abuse of notation, this represents that this operation involves all servers together.

\begin{figure*}[!t]
    \centering
    \includegraphics[width=.9\linewidth]{images/FantaSpec.jpg}
    \caption{Sequence diagram of the workflow described in Section \ref{sec:workflow}.}
    \label{fig:sequence diagram}
\end{figure*}

==> design.tex <==
\st{I would move this section just after design goals with a reference to Fig.1}

\begin{comment}%%%%%% PREVIOUS ROLE SECTION
\paragraph{Roles} 
We consider three different modules \st{components? A module is something also used in Tendermint, we mean here a Tendermint Module or it is something else? }: the federated learning, the blockchain and the distributed storage which originate the following roles.

\st{: Our system is composed of a set of nodes, separated in Learners, Model Owners and Aggregators. All the nodes are also \bcclients, i.e. able to send transactions to the blockchain. A special set of blockchain participants can  play the role of \bcvals:  a \bcval is a blockchain participant that maintains the blockchain history, collects transactions from other \bcclients and runs a BFT-Consensus protocol together with other \bcvals to validate transactions 
before adding them to the blockchain. Note that we consider a public blockchain in which each \bcclient is free to become a \bcval with the only caveat that 
in Fantastyc all the \flaggrs are also blockchain \bcvals to ensure the integrity of the whole learning process. 
---To set up any learning process in Fantastyc, a \flowner submits a model to train to the blockchain along with a rewarding policy, while \flclients can register to train the submitted model if they accept the proposed rewarding. During learning, at each learning iteration, \flclients
produce new model updates out of their local data and using the previous aggregated model, while \flaggrs produce the aggregated model out of model updates provided by \flclients. % as a model and a reward to train that model. 
All the models are registered in the blockchain through data \textit{anchoring}. Indeed for size reasons, only a cryptographic fingerprint (e.g. a hash) of the model is registered in the blockchain, alongside a reference to the external distributed storage where the model is actually stored. To guarantee Byzantine fault-tolerance of the distributed storage, Fantastyc envisages that a storage's replica is maintained by each \flaggr's node, but other deployments can be envisaged. }

%Federated learning wise, a \flowner submits models to train to the blockchain, while \flclients register themselves to train a submitted model. During learning, at each learning iteration, \flclients
%produce new model updates out of their local data and using the previous aggregated model, while \flaggrs produce the aggregated model out of model updates provided by \flclients. % as a model and a reward to train that model. 
%All the models are registered in the blockchain through data \textit{anchoring}. Indeed for size reasons, only a cryptographic fingerprint (e.g. an hash) of the model is registered in the blockchain, alongside a reference to the external distributed storage where the model is actually stored. 

%Blockchain wise, a \bcval is a blockchain node that maintains the blockchain history, collects transactions from the \bcclients and runs a BFT-Consensus algorithm to validate transactions before adding them into the blockchain. All the federated learning roles, i.e., \flaggr, \flowner and \flclient are \bcclients 

%Distributed storage wise we have the \dsreplicas that implement the distributed storage and the pub/sub middleware and the \dsclients that publish and retrieve information on the pub/sub middleware which are also stored in the distributed storage. \bcclients are also \dsclients. 
%Replicas play different sub-roles: BC-Validators are the roles devoted to the blockchain implementation. FL-Aggregators are the roles devoted to the Federated Learning process and finally DS-nodes are the roles devoted to the distributed storage implementation. Clients play different sub-roles: FL-Model providers and FL-Clients. An FL-Model Provider can issue to Fantastyc a new Federated Learning task (FL-task) and being notified when the task is over, obtaining the new trained model. FL-Clients, monitors Fantastyc for new FL-tasks and if interested, apply and (potentially) contribute for some of them. At the end of the task, FL-Clients are rewarded for their work.
\end{comment}
\adp{In the following we discuss many points, we should find a way to arrange them properly}
\paragraph{On-chain information}
For size reasons, for each federated learning process (we refer to it also as federated learning task) we record on-chain only the necessary information for tracking the process. Large size data are stored off-chain, on a distributed storage, while on-chain we store the anchor to the data. The following information are on chain:
\begin{itemize}
    \item the \flowner's initial transaction which carries the learning task specifications:
    \begin{itemize}
        \item the aggregation function
        \item the \flclients selection function
        \item the anchoring model (if any)
        \item the required accuracy level
        \item the rewarding strategy
        \item ...
    \end{itemize}
    \item \flclients's staking transactions used to self-register as learners to a on-chain published, and not yet finished, task. 
    \item for each learning iteration (which starts when there are sufficiently many \flclients available):
    \begin{itemize}
        \item a \flaggr transaction that selects \flclients along with the anchoring to the model to be trained
        \item a \flaggr transaction that determine the set of \flclients' update and score anchors to be considered for the following aggregation and evaluation respectively
        \item if the learning process is not yet finished, a \flaggr transaction that selects \flclients along with the anchoring to the new aggregated model to be trained and the aggregated score ; otherwise,  a \flaggrs closing transaction that anchors the final model and contains information useful for \flclients reward, i.e., how many times each \flclient contributed in the learning process.
    \end{itemize}
\end{itemize} 
%For each learning iteration, \flaggrs notify the selected \flclients  (only a subset of them is selected for each iteration) by recording that set on-chain along with the anchoring to the model to consider for the learning.
%\flaggrs collect models computed by selected learners and proceed to anchor a set of them in the blockchain, that set is the input for the next aggregated model. \flaggrs aggregate the values receved from \flclients and through a BFT consensus reach consensus on a common valid result, i.e. the aggregated model. The result is also anchored in the blockchain, for each iteration till the last iteration. For the last iteration \flaggrs issue the closing transaction that anchors the final model and contains information useful for \flclients reward, i.e., how many times each \flclient contributed in the learning process. 

%issue transactions containing selected \flclients for that round and the data anchoring about \flclient's updates and \flaggrs's aggregated models, both fully stored on the distributed storage. Finally; \flaggrs issue the closing transaction containing the anchoring to the final model and the information for the \flclients reward.

\paragraph{Off-chain information: Eventual Consistent Distributed Storage}
As previously described, our construction employs on-chain anchoring to track \flclients' updates and scores, and \flaggrs' aggregated models and scores. The whole data is stored off-chain on a distributed key value storage to gain scalability and efficiency. 

The blockchain and the distributed storage when combined must guarantee that, if there is some data anchored on-chain, then this data is eventually accessible on the distributed storage.
%To maintain consistency, we have implemented measures to prevent any discrepancies between the on-chain anchors and the data stored in the distributed storage. 
We use a distributed key value storage that operates under the principle of eventual consistency, meaning that any information published by a correct \dsclient will eventually be accessible to all other \dsclients.
In \fanta, we use \bcvals to ensure that any information anchored on-chain is valid (it originates from the learning process) and eventually available on the key value store. This means that although a \dsclient may not immediately access the information after it has been published on-chain, it will eventually become accessible.
Additionally, our system enforces that each key is the hash of its corresponding value. This design ensures that no existing value can be overwritten by a different one, as doing so would result in a different key. It also prevents any potential issues that may arise from concurrent write operations on the same key.


\paragraph{Off-chain computation validation}
In \fanta, three main operations are carried out off-chain: \flclients' updates computation, \flaggrs' model aggregation, and \flaggr \flclients pseudo-random selection. The first operation, which is based on \flclients' local data, cannot be validated without violating their privacy or incurring the cost of using cryptographic approaches.

Concerning the remaining operations, in \fanta, both \flaggrs and \bcvals are located on the same node. As a result, \bcvals are capable of validating the aggregated model computed by \flaggr at consensus time, even though the aggregation is conducted off-chain. 
This prevents Byzantine \flaggrs to anchor on-chain a model which does not originate from the previously selected updates. Therefore, an aggregated model stored on the distributed storage and anchored on-chain is considered valid, as it has been validated by the \bcvals. Similarly holds for the \flclients selection.

\paragraph{Block production and federated learning process asynchrony}
In the \fanta setting, the learning process evolution is dependent on when information are stored on chain. Indeed, it is used also as synchronization point among the aggregators. To go faster, \fanta does not track each \flclient update on chain (which would implies, waiting that \flaggrs delivers \flclients updates, record them on the blockchain before considering them for the new model computation), but \flaggrs anchor on chain the set of updates that will be used to aggregate the next model. In this way, \flaggr can aggregate the new model as soon as they observe that the set is anchored on chain. Hereafter, when there is new block proposal containing the anchor to the new model, \bcvals do not need to compute the aggregation at consensus time to validate the proposal, they only need to check that proposal againt the model they already computed. 

\adp{To discuss that consensus does not wait: rewrite the paragraph and discuss the two validation part: the update set and the aggreated model. Optional, add a paragraph with the naive way, that can be removed. }

\paragraph{Modularity for Flexibility}
\fanta is specifically designed to enable different and diverse learning tasks to be conducted in parallel. To achieve this, its design is highly modular, relying on a dispatcher to route information to the appropriate module. When a \flowner proposes a learning task, it specify the minimum number of \flclients to select at each round, maximum number of round for the learning process, aggregation function, client selection function, and rewarding mechanism. Additionally, new functions and mechanisms can be added to the system, making it highly flexible and adaptable to diverse learning scenarios.  


% \paragraph{FL-Task-param}
% \adp{List all the parameters, @William}
% \wb{
% \{\\
% identifier\\
% min\_clients\\
% max\_rounds\\
% aggregation\_params\\
% selection\_params\\
% training\_params\\
% \}
% }


\adp{we should understand how this can be done, it is a bit like governance, the new module should be analysed and voted to avoid problems.}


\paragraph{Clients selection}%\st{to rephrase in simple words}
For each round of a given FL-Task, a random subset of participating \flclients (clients that did stake) is selected and recorded on-chain. This subset is validated by blockchain \bcvals, indeed each of them run the selection process which is based on a pseudo-random function that takes the hash of the previous round's aggregated model and the participating \flclients as input. The function outputs a verifiable pseudo-random subset of selected \flclients.

In each round of an FL-Task, a random subset of participating \flclients (clients that did stake) is selected and recorded on-chain. This subset is validated by blockchain \bcvals, who use a pseudo-random function based on the previous round's aggregated model and the participating \flclients to output a verifiable pseudo-random subset of selected \flclients.

% Let $Clients_{FL-Task\_ID}$ be the set of \flclients that manifested interest in participating to the considered FL-Task $FL-Task\_ID$. For each FL-Task $FL-Task$, at each round $r$, a random subset of \flclients is selected from $Clients_{FL-Task\_ID}$. Such subset is recorded on-chain. As discussed in the previous paragraph, information (which can be the result of a computation) recorded on-chain have to be validated by \bcvals. To this aim, the subset of \flclients is the result of a pseudo-random function. 
% The function $Select\_Clients$ takes as input seed the hash of the aggregated model resulting from the previous round $r-1$ for the same $FL-Task$\footnote{\adp{we are not able to assess if using the hash of the last aggregated model is equivalent or not with using the hash of the blockchain}} and $Clients_{FL-Task\_ID}$. $Select\_Clients$ outputs a pseudo-random sampling out of $Clients_{FL-Task\_ID}$. Such a result if verifiable by any \bcval.

\paragraph{On determinism and non-determinism}
\adp{explain the need for determinism in the blockchain context and the two problems of aggregating the model, which is expressed in floating points and the pseudo-random functions as the client selection}

\paragraph{Pub/Sub vs Pub/BC/Query}\adp{not sure we need this section}
{\bf draft} The first is faster, the second reduces the amount of new model messages that \flclients receive. Moreover, the query is issued after the message has been announced on the blockchain, which implies the \bcvals validation (no spam). 
In any case, we can implement both, the feeling is that the second one might performing better when there are many \flclients and many FL-Tasks in parallel, which might imply the network saturation. However, we would need to carry out experiments to have a more clear idea.
In any case, we might let the \flowner specify which approach to follow and in case pay different amounts depending on it. Lastly, the Pub/BC/Query is auditable-friendly with respect to the distributed storage.



\paragraph{BFT Aggregation functions}
\am{cite median, trimmed mean, Krum and RLR}


\paragraph{Privacy-preserving Mechanism}
\st{put here a paragraph on how we envisage to protect from Model Inversion}

\paragraph{Solution}
In the following we discuss how all those mechanisms concur in providing the design goals. \adp{draft}
\begin{itemize}
\item \textbf{Security}: our scheme is robust against Byzantine \flclients thanks to BFT aggregation function and against Byzantine \flaggrs thanks to the consensus validity which prevents them to record invalid information on-chain. 
\item \textbf{Privacy}: \flclients privacy is obtained thanks to the privacy-preserving mechanisms... \adp{I let Aurelien complet this part :)}
\item \textbf{Scalability}: thanks to the pub/sub middleware, the asynchrony between the consensus and the information dissemination our scheme is efficient whatever the size of the federated model and the number of clients. 
\end{itemize}



==> images/seqDiagram.tex <==
\newcommand{\SMR}{\ensuremath{\text{SMR}}}
\newcommand{\CLIENT}{\ensuremath{\text{client}}}
\newcommand{\HASH}[1]{\ensuremath{H({#1})}}
\newcommand{\cmdApply}{\ensuremath{\bullet}}
\newcommand{\msgSMR}[1]{\ensuremath{{#1}^\SMR}}

\newcommand{\MO}{\ensuremath{\text{Model Owner}}}
\newcommand{\LEARNER}{\ensuremath{\text{Learner}}}
\newcommand{\STORAGE}{\ensuremath{\text{DS}}}
\newcommand{\AGG}{\ensuremath{\text{Agg}}}


\newcommand{\newFL}{\ensuremath{\text{NEW\_FL\_TASK}}}
\newcommand{\newStake}{\ensuremath{\text{STAKE}}}
\newcommand{\readStake}{\ensuremath{\text{READ\_STAKE}}}
\newcommand{\msgSMRLocal}[1]{\ensuremath{{{#1}_\text{Local}^\SMR}}}
\newcommand{\msgAGG}[1]{\ensuremath{{#1}^\AGG}}
\newcommand{\msgStartFL}{\ensuremath{\text{START\_FL\_TASK}}}
\newcommand{\msgStartRound}{\ensuremath{\text{START\_FL\_ROUND}}}
\newcommand{\msgStoreModel}{\ensuremath{\text{STORE\_MODEL}}}
\newcommand{\msgCheckSelected}{\ensuremath{\text{READ\_CHECK\_SELECTED}}}
\newcommand{\queryDS}{\ensuremath{\text{QUERY\_DS} (\HASH{model})^\STORAGE}}


\tikzset{every picture/.append style={transform shape,font=\scriptsize, scale=0.9}}
\begin{sequencediagram}

    \pgfumlsdunderlinefalse
    \newthread{MO}{\shortstack{
        \begin{tikzpicture}
          \node [copy shadow,fill=blue!20,draw=black,thick,align=center] {Model\\ Owner};
        \end{tikzpicture}}
                  }{}
  %\newthread{MO}{Model Owner}

    \newthread{LN}{\shortstack{
    %\newthread{LN}{\shortstack{Client\\ \\
        \begin{tikzpicture}
          \node [copy shadow,fill=blue!20,draw=black,thick,align=center] {Learner};
        \end{tikzpicture}}
                  }{}

    \newinst[3]{APP}{\shortstack{$\text{SMR}$\\ \\ 
    \begin{tikzpicture}
      \node [copy shadow, fill=green!20,draw=black,thick ,align=center] {Tendermint};
    \end{tikzpicture}}
              }{}

    \newinst[1]{AGG}{\shortstack{Aggregators\\ \\ 
    \begin{tikzpicture}
      \node [copy shadow, fill=green!20,draw=black,thick ,align=center] {TensorFlow};
    \end{tikzpicture}}
              }{}

    \newinst[1]{DS}{\shortstack{Distributed \\ Storage \\
    \begin{tikzpicture}[shape aspect=.5]
      \tikzset{every node/.style={cylinder, shape border rotate=90, draw,fill=green!25}}
      \node[copy shadow]  at (1.5,0) {Zenoh};
    \end{tikzpicture}}
                  }{}    
% \begin{tikzpicture}
%    \draw[dotted] (0,0) rectangle (2,2);
% \end{tikzpicture}

    \begin{call}{MO}{$T:$ \msgSMR{\newFL}}{APP}{}
    \begin{call}{APP}{Consensus($T$)}{APP}{$App \cmdApply T$} \end{call}

    %\begin{messcall}{APP}{event}{MO}{} \end{messcall}
    %\begin{messcall}{APP}{event}{LN}{} \end{messcall}

    \mess{APP}{Event}{MO}
    \mess{APP}{Event}{LN}
    \end{call}

    \begin{call}{LN}{$R:$ \msgSMR{\text{READ\_}\newFL}}{APP}{$App[R]$}
        \begin{call}{APP}{Consensus($R$)}{APP}{$App \cmdApply R$} \end{call}
    \end{call}

    \begin{call}{LN}{$S:$ \msgSMR{\newStake}}{APP}{}
        \begin{call}{APP}{Consensus($S$)}{APP}{$App \cmdApply S$} \end{call}
    \end{call}
 
    \mess{APP}{Event}{AGG}
    \begin{sdblock}{While($App[T_{id}][\newStake]) \leq k$)}{}
      \begin{call}{AGG}{$\msgSMRLocal{\readStake}$}{APP}{}\end{call}
    \end{sdblock}

    \begin{call}[2]{AGG}{startFL$(T_{id},model,round)$}{AGG}{} \end{call}
    \begin{call}{AGG}{$\msgStoreModel(T_{id},model,round)$}{DS}{\HASH{model}} \end{call}

    \begin{call}{AGG}{$SR:$ $\msgSMR{\msgStartRound}(T_{id},\HASH{model}, round,Learners)$}{APP}{}
        \begin{call}{APP}{Consensus($SR$)}{APP}{$App \cmdApply SR$} \end{call}
    \mess{APP}{Event}{LN}
    \end{call}

    \begin{call}{LN}{$CS:$ \msgSMR{\msgCheckSelected}}{APP}{$L_{id} \in App[CS]$}
        \begin{call}{APP}{Consensus($CS$)}{APP}{$App \cmdApply CS$} \end{call}
    \end{call}

    \begin{call}{LN}{$M:$ \queryDS}{DS}{$model$}
      \begin{call}{DS}{Fetch(\HASH{model})}{DS}{} \end{call}
    \end{call}

    \begin{call}{LN}{produceUpdate($model,\text{local data}$)}{LN}{$\text{new model}$} \end{call}
\end{sequencediagram}


==> implementation.tex <==
% \begin{figure*}[h]
%   \includegraphics[width=\textwidth]{light_spec2.JPG}
%   \caption{The figure show the communication solution steps omitting the computational ones, described in the text. In particular, messages that pass through the pub/sub middlewere are depicted in blue and in blue we highlight the topic associated to the message. Messages (blockchain transaction) that passes through the p2p network and aims at being recorded on the blockchain are depicted in green. \adp{WIP, the figure consider pub/sub paradigm and not pub/bc/query, add the evaluation part}}\label{fig:spec}
% \end{figure*}


Figure \ref{fig:seq} describes the main Fantastyc functioning in how the \flowner, \flclient and \flaggrs interact. In particular in the latter, we describe also the different modules interaction: blockchain, distributed storage and \flaggr.

The communication between \flowners, \flclients and \flaggrs is performed via a publish and subscriber middleware, however they also communicate indirectly recording information (or their anchor) in the blockchain.

The communication between \flowners, \flclients, and \flaggrs is facilitated through a publish and subscribe middleware, which allows for direct communication between the parties. However, they also communicate indirectly by recording information and anchors on the blockchain. This approach provides an additional layer of security and transparency to the communication process, as by recording information on the blockchain, the parties involved can verify the information validity.

\fanta is designed to run different FL-Tasks in parallel, however, here in the following we describe a single FL-Task process. In Figure \ref{fig:seq} the \flowner records on the blockchain the announce for a new FL process (1). \flclients listen to the blockchain and retrieve the new task (2), evaluate it, and decide whether to participate in the task by staking (3) based the rewarding policy. 
Once enough \flclients have joined (4), the \flaggrs start a new round (5,6) by selecting a subset of participants and storing the model for the next learning round on the distributed storage (5) while recording the anchor to it and the list of selected \flclients on the blockchain (6).
\adp{I am here with the modiffs.}
The Figure details for each \dsclient, the topics at which it is subscribed \adp{To modify here depending on the paradigm that we follow}. For the sake of simplicity, in Figure \ref{fig:spec} nor in the following description we detail the \flclients steps when a \flclient as \bcclient retrieves information from the blockchain neither the message retrieve from the distributed storage as \dsclient. We consider that \flclients are subscribed to a \bcval \adp{it would be more precise to say full-blockchain node, but since we have a fixed committee we might semplify that} to be notified about Blockchain events. 

In the following we say that a \bcclient publishes a message meaning that that this message has an associated topic and is eventually recorded in the distributed key value store, having as key the message hash. Moreover, if there are \bcclients subscribed to that topic, they are notified and receive that message automatically.

The communication between \bcvals and \bcclients is performed via a peer to peer network \adp{check the system model}.
We identify as $\langle TAG, field_1, field_2, \dots, field_m \rangle$ the blockchain transactions, signed by the emitter (in green in the Figure). 

In the following we say that \bcclient issues a transaction, which means that he sends that transaction to a \bcval  (by assumption each \bcclient is connected to one correct \bcval) which checks the transaction validity before appending it in his memPool and diffusing it to the other \bcvals. We consider that eventually, if valid, such transaction is inserted in a block proposal successfully decided (appended to the blockchain). 

Let us note that, when information are published on Zenoh, their anchoring is also recorded on the blockchain via blockchain anchoring transactions. \bcvals, when producing a block, considers only anchoring transactions for information that they observed as published on Zenoh.

\adp{In the follow, double check that the validity verifications are well explicited.}

% \textbf{Each time a message is published on the pub/sub middleware, the message is also stored in the distributed storage}. The distributed storage is a key value store such that the key of the value \textbf{must} be the hash of that value. This can be directly enforced by the DS when a new value is stored, if not, the DS must verify that the pair value, key is such that the key is the hash of the value. 

\paragraph{Single FL-Task processing.} An FL-Task, started by an \flowner, is processed as in the steps partially depicted in Figure~\ref{fig:spec}, which we fully describe below.
We use the following syntax.    

\noindent\textbf{1.} An \flowner aiming at starting a new FL-Task with a predefined model to train \adp{not sure it is the right terminology} publishes that model before anchoring it on-chain (next step). If there is not a predefined model, the \flowner moves directly to the next step.
 
\noindent\textbf{2.} The \flowner issues a blockchain transaction $\mathrm{NEW\_TASk}$ containing the task identifier $\mathrm{task\_id}$, the task parameters $\mathrm{task\_param}$ (this field contains all the FL-Task parameters, the bonded rewarding amount for FL-Clients and BC-Validators and the rewarding strategy) and finally the model $\mathrm{model}$ (if any). 

\noindent\textbf{3.} 
When a \flclient observes in the blockchain a new $\mathrm{NEW\_TASk}$ and he is willing to participate, he moves to step 4. If that transaction is referring to the hash of a model, then the \flclient first has to retrieve it or wait to have it. \adp{it will depend on the chosen pattern.}

\noindent\textbf{4.} \flclient interested in participating to an on-going FL-Task $\mathrm{FL\_Task\_ID}$ issues a $\mathrm{STAKE}$ transaction to signal the amount of stake $S$ that they stake to be considered to the FL-Task $\mathrm{FL\_Task\_ID}$ \adp{such stake should overcome a threshold}, (which amount is defined in $\mathrm{FL\_task\_param}$).

\noindent\textbf{5.} before moving to step 6, \flaggrs wait to collect $min\_clients$ $\mathrm{STAKE}$ transactions issued at step 4 for $max\_block$ blocks ($min\_clients$ and $max\_block$ are defined in $\mathrm{FL\_task\_param}$) after the block containing the $\mathrm{NEW\_TASk}$ transaction \adp{it can also be true that the aggr just wait and then go with the clients that they collected}.

\noindent\textbf{7.} if the FL-Task $FL\_Task\_ID$ is on-going, then the \flaggrs publish a message having as topics $\mathrm{NEW\_MODEL}$ the specific $\mathrm{FL\_Task\_ID}$, the specific round $\mathrm{r}$ and $\mathrm{model}$ and as payload the model.  If $FL\_Task\_ID$ is finished, then the \flaggrs publish the final model. 

\noindent\textbf{6.} At the step, \flaggrs confirms on the blockchain what they published on Zenoh in the previous step. If FL-Task is no yet finished, they issue a transaction $\mathrm{NEW\_TASk}$ with the list of selected clients $\mathrm{selected~clients}$ along with the hash of model for the next round.
Such transaction is valid if $\mathrm{selected~clients}$ is valid, i.e., it is the result of the pseudo-random function $Select\_clients$. Concerning the hash of the new model, such transaction is valid during the first round only if the new model is compliant with the content of $\mathrm{NEW\_TASk}$ transaction. For the later rounds, such a transaction is valid only if the new aggregated model is compliant with the agreed set of \flclients updated coming from the previous round $S_{r-1}$, defined later at step 11.
If $FL\_Task\_ID$ is finished, then the \flaggrs issue the Closing Transaction $\mathrm{CT}$, to deliver the finalized model, and finally to state how much each \flclients contributed to the learning process, which determines the reward repatriation.


\noindent\textbf{8.} \flclients are subscribed to $\mathrm{NEW\_MODEL}$ topic, so eventually they receive the model \adp{to change accordingly with the paradigm that we chose}. When \flclients observe that they are selected and they got the model for that round, then they can produce the update.

\noindent\textbf{9.} when finished, \flclients publish their update labelled with the topics $\mathrm{UPDATE}$, and the relative FL-Task and round, $\mathrm{FL\_Task\_ID}$ $\mathrm{r}$.


\noindent\textbf{10.} \flaggrs are subscribed to the UPDATE topic and wait sufficiently many updates for the current round $r$ from the selected clients for a certain number of blocks from the publication of the last new model (parameters defined in $\mathrm{FL\_task\_param}$).


\noindent\textbf{11.} When a \flaggr collects sufficiently many updates, he issues a $\mathrm{UPDATES\_SET}$ transaction to propose $selected\_updates$ a set of updates (in the form of their hashes) for the round $r$ as the updates to be considered to aggregate the next model. %$\langle\mathrm{UPDATES\_SET}, \mathrm{FL\_Task\_ID}, \mathrm{r}, \mathrm{S_r}\rangle$. \adp{update the Figure accordingly} % which contains the hashes of each updates that the A/V wants to consider to produce the next model for a particular FL-Task $\mathrm{FL\_Task\_ID}$ at round $\mathrm{r}$.
%
%At BC-Validator side, such a transaction can be inserted in a proposal block and endorsed only if the BC-Validator has been notified with all the updates in $S_r$. 
%then he publishes on the blockchain the following transaction \\


\noindent\textbf{12.}
At \bcval side, such a transaction can be inserted in a proposal block and endorsed only if the \bcvals have been notified with all the updates in $selected\_updates$. 
%Finally, A/V when observing a transaction 11 in the block proposal, they verify that they observed all the updates proposed, if not, they reject the block.
For each $\mathrm{FL\_Task}$ and for each $r$, only one transaction is admitted in the blockchain, which determines the next model. At this point go to step 6, where the \flaggrs compute and publish the next model. %and publish it and a new transaction with the selected FL-Clients to continue the loop.



==> relatedWork.tex <==
\begin{table}[htb]
\boldmath
\center
   \begin{tabular}{ c || c | c  | c }
      & Security & Privacy & Scalability \\ 
     Biscotti \cite{biscotti20} & \ding{51} & \ding{51} & \ding{55} \\ 
     - & - & - & - \\ 
   \end{tabular}
\unboldmath 
\caption{Main features of state-of-the-art BC-based federated learning approches}
\label{tab:feat}
\end{table}


==> solution.tex <==
In the following we describe how the \fanta components interact to train a new model, from the moment the \flowner starts the task until the task is accomplished. As depicted in the sequence diagram in Figure~\ref{fig:seq}, we consider the \flowner, the \flclient and the \bcval, which contains on the same node, a \bcclient, a \dsreplica and an \flaggr module. 

==> solutionExt.tex <==
\begin{figure*}[h]
  \includegraphics[width=\textwidth]{light_spec2.JPG}
  \caption{The figure show the communication solution steps omitting the computational ones, described in the text. In particular, messages that pass through the pub/sub middlewere are depicted in blue and in blue we highlight the topic associated to the message. Messages (blockchain transaction) that passes through the p2p network and aims at being recorded on the blockchain are depicted in green. \adp{WIP, the figure consider pub/sub paradigm and not pub/bc/query, add the evaluation part}}\label{fig:spec}
\end{figure*}


Figure \ref{fig:spec} describes the main Fantastyc functioning in integrating the FL process with the Blockchain and the distributed storage. 

\paragraph{Preliminaries.} \fanta is designed to run different FL-Tasks in parallel, however, here in the following we describe a single FL-Task processing. 

The communication between \flowners, \flclients and \flaggrs is performed via a publish and subscriber middleware. In Figure \ref{fig:spec} we identify those communications with blue colors. % arrows and we let the key word PUB precede the message. %The first parameters of the message, in blue color, represent the topics in which the publisher is publishing. In particular, we identify as $PUB(\langle topic_1, topic_2, \dots, topic_n, payload \rangle)$ the messages for the distributed storage. The last argument is the messages payload and the first ones identify the topic (expressed as a topics and sub topics, in blue in the Figure). The whole message is signed by the published. 

The Figure details for each \dsclient, the topics at which it is subscribed \adp{To modify here depending on the paradigm that we follow}. For the sake of simplicity, in Figure \ref{fig:spec} nor in the following description we detail the \flclients steps when a \flclient as \bcclient retrieves information from the blockchain neither the message retrieve from the distributed storage as \dsclient. We consider that \flclients are subscribed to a \bcval \adp{it would be more precise to say full-blockchain node, but since we have a fixed committee we might semplify that} to be notified about Blockchain events. 

In the following we say that a \bcclient publishes a message meaning that that this message has an associated topic and is eventually recorded in the distributed key value store, having as key the message hash. Moreover, if there are \bcclients subscribed to that topic, they are notified and receive that message automatically.

The communication between \bcvals and \bcclients is performed via a peer to peer network \adp{check the system model}.
We identify as $\langle TAG, field_1, field_2, \dots, field_m \rangle$ the blockchain transactions, signed by the emitter (in green in the Figure). 

In the following we say that \bcclient issues a transaction, which means that he sends that transaction to a \bcval  (by assumption each \bcclient is connected to one correct \bcval) which checks the transaction validity before appending it in his memPool and diffusing it to the other \bcvals. We consider that eventually, if valid, such transaction is inserted in a block proposal successfully decided (appended to the blockchain). 

Let us note that, when information are published on Zenoh, their anchoring is also recorded on the blockchain via blockchain anchoring transactions. \bcvals, when producing a block, considers only anchoring transactions for information that they observed as published on Zenoh.

\adp{In the follow, double check that the validity verifications are well explicited.}

% \textbf{Each time a message is published on the pub/sub middleware, the message is also stored in the distributed storage}. The distributed storage is a key value store such that the key of the value \textbf{must} be the hash of that value. This can be directly enforced by the DS when a new value is stored, if not, the DS must verify that the pair value, key is such that the key is the hash of the value. 

\paragraph{Single FL-Task processing.} An FL-Task, started by an \flowner, is processed as in the steps partially depicted in Figure~\ref{fig:spec}, which we fully describe below.
We use the following syntax.    

\noindent\textbf{1.} An \flowner aiming at starting a new FL-Task with a predefined model to train \adp{not sure it is the right terminology} publishes that model before anchoring it on-chain (next step). If there is not a predefined model, the \flowner moves directly to the next step.
 
\noindent\textbf{2.} The \flowner issues a blockchain transaction $\mathrm{NEW\_TASk}$ containing the task identifier $\mathrm{task\_id}$, the task parameters $\mathrm{task\_param}$ (this field contains all the FL-Task parameters, the bonded rewarding amount for FL-Clients and BC-Validators and the rewarding strategy) and finally the model $\mathrm{model}$ (if any). 

\noindent\textbf{3.} 
When a \flclient observes in the blockchain a new $\mathrm{NEW\_TASk}$ and he is willing to participate, he moves to step 4. If that transaction is referring to the hash of a model, then the \flclient first has to retrieve it or wait to have it. \adp{it will depend on the chosen pattern.}

\noindent\textbf{4.} \flclient interested in participating to an on-going FL-Task $\mathrm{FL\_Task\_ID}$ issues a $\mathrm{STAKE}$ transaction to signal the amount of stake $S$ that they stake to be considered to the FL-Task $\mathrm{FL\_Task\_ID}$ \adp{such stake should overcome a threshold}, (which amount is defined in $\mathrm{FL\_task\_param}$).

\noindent\textbf{5.} before moving to step 6, \flaggrs wait to collect $min\_clients$ $\mathrm{STAKE}$ transactions issued at step 4 for $max\_block$ blocks ($min\_clients$ and $max\_block$ are defined in $\mathrm{FL\_task\_param}$) after the block containing the $\mathrm{NEW\_TASk}$ transaction \adp{it can also be true that the aggr just wait and then go with the clients that they collected}.

\noindent\textbf{7.} if the FL-Task $FL\_Task\_ID$ is on-going, then the \flaggrs publish a message having as topics $\mathrm{NEW\_MODEL}$ the specific $\mathrm{FL\_Task\_ID}$, the specific round $\mathrm{r}$ and $\mathrm{model}$ and as payload the model.  If $FL\_Task\_ID$ is finished, then the \flaggrs publish the final model. 

\noindent\textbf{6.} At the step, \flaggrs confirms on the blockchain what they published on Zenoh in the previous step. If FL-Task is no yet finished, they issue a transaction $\mathrm{NEW\_TASk}$ with the list of selected clients $\mathrm{selected~clients}$ along with the hash of model for the next round.
Such transaction is valid if $\mathrm{selected~clients}$ is valid, i.e., it is the result of the pseudo-random function $Select\_clients$. Concerning the hash of the new model, such transaction is valid during the first round only if the new model is compliant with the content of $\mathrm{NEW\_TASk}$ transaction. For the later rounds, such a transaction is valid only if the new aggregated model is compliant with the agreed set of \flclients updated coming from the previous round $S_{r-1}$, defined later at step 11.
If $FL\_Task\_ID$ is finished, then the \flaggrs issue the Closing Transaction $\mathrm{CT}$, to deliver the finalized model, and finally to state how much each \flclients contributed to the learning process, which determines the reward repatriation.


\noindent\textbf{8.} \flclients are subscribed to $\mathrm{NEW\_MODEL}$ topic, so eventually they receive the model \adp{to change accordingly with the paradigm that we chose}. When \flclients observe that they are selected and they got the model for that round, then they can produce the update.

\noindent\textbf{9.} when finished, \flclients publish their update labelled with the topics $\mathrm{UPDATE}$, and the relative FL-Task and round, $\mathrm{FL\_Task\_ID}$ $\mathrm{r}$.


\noindent\textbf{10.} \flaggrs are subscribed to the UPDATE topic and wait sufficiently many updates for the current round $r$ from the selected clients for a certain number of blocks from the publication of the last new model (parameters defined in $\mathrm{FL\_task\_param}$).


\noindent\textbf{11.} When a \flaggr collects sufficiently many updates, he issues a $\mathrm{UPDATES\_SET}$ transaction to propose $selected\_updates$ a set of updates (in the form of their hashes) for the round $r$ as the updates to be considered to aggregate the next model. %$\langle\mathrm{UPDATES\_SET}, \mathrm{FL\_Task\_ID}, \mathrm{r}, \mathrm{S_r}\rangle$. \adp{update the Figure accordingly} % which contains the hashes of each updates that the A/V wants to consider to produce the next model for a particular FL-Task $\mathrm{FL\_Task\_ID}$ at round $\mathrm{r}$.
%
%At BC-Validator side, such a transaction can be inserted in a proposal block and endorsed only if the BC-Validator has been notified with all the updates in $S_r$. 
%then he publishes on the blockchain the following transaction \\


\noindent\textbf{12.}
At \bcval side, such a transaction can be inserted in a proposal block and endorsed only if the \bcvals have been notified with all the updates in $selected\_updates$. 
%Finally, A/V when observing a transaction 11 in the block proposal, they verify that they observed all the updates proposed, if not, they reject the block.
For each $\mathrm{FL\_Task}$ and for each $r$, only one transaction is admitted in the blockchain, which determines the next model. At this point go to step 6, where the \flaggrs compute and publish the next model. %and publish it and a new transaction with the selected FL-Clients to continue the loop.

%\adp{I am here ################ what is after, I didn't revise yet.}

\paragraph{Discussion on performances.}
The specification design is such that the new model is not computed, nor verified (if possible) at consensus time. First, FL-Aggregators agree on the set of updates to consider to compute the new model. Second, FL-Aggregators compute the new model. Third, they publish it and issue a transaction with the hash of it. FL-Validators already computed the new model, hence BC-Validators at consensus time can quickly verify if the hash of the new model candidate to be stored into the blockchain is valid or not.  However, if a BC-Validator did not obtained the updates sufficiently early, then it might either refuse of be obliged to compute the new model at consensus time. We will verify that at evaluation time and if necessary we might force some blocks delay in between the set of updates and the new model publications on the blockchain.

\paragraph{Correctness discussion.} In this paragraph we provide an informal discussion on the correctness of the provided solution. In the following we focus on two aspects: the auditability of the FL-process (i.e., the capability for an auditor to reconstruct the FL-process) and the FL-process liveness (i.e., each FL-Task terminates). 

The \textbf{auditability} is given by the information stored into the blockchain. As discussed before, for confidentiality and space complexity reasons, most of the information are stored off-chain, letting only a trace of those in the blockchain. 

In Fantastyc, for auditability reasons, we aim at reflecting the content of the DS in the blockchain. More into details, the blockchain contains the hashes of the values that are stored stored into the DS. A natural way to enforce it, is to write on the blockchain the hash of a value once that value is written in the DS, such that if the hash of a value is on the blockchain, then it is possible to retrieve the corresponding value on the DS (whose key is the hash). We refer to that as \textbf{atomicity}. 

To avoid waiting that a value is written in the DS before trace it on the blockchain, in the following we require that an actor writes the hash of a value on the blockchain after that such a value has been published on the middle-ware. From the eventual consistency property of the middleware, we know that eventually all the subscribed actors will get notified for that message. Hence there is no reason to wait for the message to be stored on the DS (liveness is guaranteed). However, nothing would prevent a Byzantine FL-Aggregator to insert on the blockchain the hash of a value that does not exist. However, the messages traced on the blockchain are: $\mathrm{NEW\_FL\_TASK}$, $\mathrm{UPDATE}$ and $\mathrm{NEW\_MODEL}$ $(\mathrm{CT})$. In all that cases, BC-Validators do not accept the transaction that that contains the hash of those values, if they did not observed the value yet. This means that, if BC-Validators got notified faster than FL-Clients for a $\mathrm{NEW\_MODEL}$, then the FL-Client might observe the trace of the new model on the blockchain but not be able to retrieve the value yet. However, we can guarantee that eventually all FL-Clients will get notified. In other words,  if the hash of a value is on the blockchain, then \textbf{eventually} it is possible to retrieve the corresponding value on the DS (whose key is the hash).  We refer to that as \textbf{eventual atomicity}.


Concerning the \textbf{liveness}, we consider the case in which the FL-process would terminate in the centralized case, i.e., there are sufficiently many clients and their data are such that eventually the FL process terminates (or, it simply terminates after a maximum number of rounds). So here in the following we discuss that the FL-Aggregators are able to collect the FL-Clients updates, when there are sufficiently many, aggregate them in a set and commit on it on the Blockchain. Finally, also commit on the blockchain about the new model and the selected clients so that a new round can start. 

FL-Clients and FL-Aggregators communicate via a pub/sub middleware that enforces eventual consistency. Hence (assuming that all FL-Aggregators are subscribed to the UPDATE topic), all FL-Aggregators are eventually notified with the produced updates. So if an FL-Aggregators receives the updates faster than the others, it can propose a transaction with a set of them for the new model, let us call it $\mathrm{tx_{set}}$. $\mathrm{tx_{set}}$ is rejected by any BC-Validator as long as the FL-Aggregator on the same node does not get all the selected updates. Eventually all FL-Aggregators will get the published updates, hence it is enough that when an FL-Aggregator produces a $\mathrm{tx_{set}}$, it has to re-issue $\mathrm{tx_{set}}$ as long as there is not transaction of the same type on the blockchain for the same FL-Task and the same round. 

Finally we discuss about the transaction that refers to the new model. Such model has to be consistent with the set of updates in $\mathrm{tx_{set}}$. Since such transaction in on the Blockchain, it means that enough correct nodes validated it, hence eventually all nodes collect the selected updates and can produce the new model, issue and/or validate it. 

